Finite Family Groups for Fermionic and Leptoquark Mixing Patterns

We employ a bottom-up and model-independent technique to search for non-Abelian discrete flavour symmetries capable of predicting viable CKM and PMNS matrices alongside of special patterns of leptoquark couplings. In particular, we analyze patterns derived when an ultra-violet flavour theory is assumed to break to global Abelian symmetries in Standard Model fermion masses and new Yukawa-like terms sourced by the leptoquark representation. The phenomenology of different classes of these `simplified models' can be explored without reference to explicit model-building assumptions, e.g. the nature of flavour symmetry breaking or any additional field content associated to it, and are also capable of explaining hints of lepton non-universality in $\mathcal{R}_{K^{(\star)}}$. Assuming experimentally interesting CKM and PMNS matrix elements, our algorithm finds an abundance of predictive non-Abelian flavour groups and therefore provides promising directions for future model building in the flavoured leptoquark space, regardless of whether the anomalous $\mathcal{R}_{K^{(\star)}}$ measurements withstand further experimental scrutiny.

==> biblioLQscan.tex <==
%INSPIRE NON-STANARD ENTRIES:


%\cite{Moriond2019}
%\bibitem{Moriond2019}
%T. Humair, talk at 2019 Rencontres de Moriond, Electroweak Interactions and Unified Theories, http://moriond.in2p3.fr/2019/EW

%BEGIN BIBLIOGRAPHY:

 


%\cite{Esteban:2018azc}
\bibitem{Esteban:2018azc}
  I.~Esteban, M.~C.~Gonzalez-Garcia, A.~Hernandez-Cabezudo, M.~Maltoni and T.~Schwetz,
  %``Global analysis of three-flavour neutrino oscillations: synergies and tensions in the determination of $\theta_23, \delta_CP$, and the mass ordering,''
  JHEP {\bf 1901} (2019) 106
  doi:10.1007/JHEP01(2019)106
  [arXiv:1811.05487 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP01(2019)106;%%
  %183 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Aaij:2019wad}
\bibitem{Aaij:2019wad}
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Search for lepton-universality violation in $B^+\to K^+\ell^+\ell^-$ decays,''
  Phys.\ Rev.\ Lett.\  {\bf 122} (2019) no.19,  191801
  doi:10.1103/PhysRevLett.122.191801
  [arXiv:1903.09252 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.122.191801;%%
  %81 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Aaij:2017vbb}
\bibitem{Aaij:2017vbb}
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Test of lepton universality with $B^{0} \rightarrow K^{*0}\ell^{+}\ell^{-}$ decays,''
  JHEP {\bf 1708} (2017) 055
  doi:10.1007/JHEP08(2017)055
  [arXiv:1705.05802 [hep-ex]].
  %%CITATION = doi:10.1007/JHEP08(2017)055;%%
  %486 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Albrecht:2018frt}
\bibitem{Albrecht:2018frt}
  J.~Albrecht [LHCb Collaboration],
  %``Lepton Flavour Universality tests with B decays at LHCb,''
  arXiv:1805.06243 [hep-ex].
  %%CITATION = ARXIV:1805.06243;%%
  %1 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Hiller:2003js}
\bibitem{Hiller:2003js}
  G.~Hiller and F.~Kruger,
  %``More model-independent analysis of $b \to s$ processes,''
  Phys.\ Rev.\ D {\bf 69} (2004) 074020
  doi:10.1103/PhysRevD.69.074020
  [hep-ph/0310219].
  %%CITATION = doi:10.1103/PhysRevD.69.074020;%%
  %383 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Bordone:2016gaq}
\bibitem{Bordone:2016gaq}
  M.~Bordone, G.~Isidori and A.~Pattori,
  %``On the Standard Model predictions for $R_K$ and $R_{K^*}$,''
  Eur.\ Phys.\ J.\ C {\bf 76} (2016) no.8,  440
  doi:10.1140/epjc/s10052-016-4274-7
  [arXiv:1605.07633 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-016-4274-7;%%
  %222 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Hiller:2014yaa}
\bibitem{Hiller:2014yaa}
  G.~Hiller and M.~Schmaltz,
  %``$R_K$ and future $b \to s \ell \ell$ physics beyond the standard model opportunities,''
  Phys.\ Rev.\ D {\bf 90} (2014) 054014
  doi:10.1103/PhysRevD.90.054014
  [arXiv:1408.1627 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.054014;%%
  %277 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Capdevila:2017bsm}
\bibitem{Capdevila:2017bsm}
  B.~Capdevila, A.~Crivellin, S.~Descotes-Genon, J.~Matias and J.~Virto,
  %``Patterns of New Physics in $b\to s\ell^+\ell^-$ transitions in the light of recent data,''
  JHEP {\bf 1801} (2018) 093
  doi:10.1007/JHEP01(2018)093
  [arXiv:1704.05340 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP01(2018)093;%%
  %289 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Altmannshofer:2017yso}
\bibitem{Altmannshofer:2017yso}
  W.~Altmannshofer, P.~Stangl and D.~M.~Straub,
  %``Interpreting Hints for Lepton Flavor Universality Violation,''
  Phys.\ Rev.\ D {\bf 96} (2017) no.5,  055008
  doi:10.1103/PhysRevD.96.055008
  [arXiv:1704.05435 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.96.055008;%%
  %209 citations counted in INSPIRE as of 06 Oct 2019


%\cite{DAmico:2017mtc}
\bibitem{DAmico:2017mtc}
  G.~D'Amico, M.~Nardecchia, P.~Panci, F.~Sannino, A.~Strumia, R.~Torre and A.~Urbano,
  %``Flavour anomalies after the $R_{K^*}$ measurement,''
  JHEP {\bf 1709} (2017) 010
  doi:10.1007/JHEP09(2017)010
  [arXiv:1704.05438 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP09(2017)010;%%
  %212 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Hiller:2017bzc}
\bibitem{Hiller:2017bzc}
  G.~Hiller and I.~Nisandzic,
  %``$R_K$ and $R_{K^{\ast}}$ beyond the standard model,''
  Phys.\ Rev.\ D {\bf 96} (2017) no.3,  035003
  doi:10.1103/PhysRevD.96.035003
  [arXiv:1704.05444 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.96.035003;%%
  %166 citations counted in INSPIRE as of 06 Oct 2019



%\cite{Ciuchini:2017mik}
\bibitem{Ciuchini:2017mik}
  M.~Ciuchini, A.~M.~Coutinho, M.~Fedele, E.~Franco, A.~Paul, L.~Silvestrini and M.~Valli,
  %``On Flavourful Easter eggs for New Physics hunger and Lepton Flavour Universality violation,''
  Eur.\ Phys.\ J.\ C {\bf 77} (2017) no.10,  688
  doi:10.1140/epjc/s10052-017-5270-2
  [arXiv:1704.05447 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-017-5270-2;%%
  %180 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Alok:2017sui}
\bibitem{Alok:2017sui}
  A.~K.~Alok, B.~Bhattacharya, A.~Datta, D.~Kumar, J.~Kumar and D.~London,
  %``New Physics in $b \to s \mu^+ \mu^-$ after the Measurement of $R_{K^*}$,''
  Phys.\ Rev.\ D {\bf 96} (2017) no.9,  095009
  doi:10.1103/PhysRevD.96.095009
  [arXiv:1704.07397 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.96.095009;%%
  %120 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Ciuchini:2019usw}
\bibitem{Ciuchini:2019usw}
  M.~Ciuchini, A.~M.~Coutinho, M.~Fedele, E.~Franco, A.~Paul, L.~Silvestrini and M.~Valli,
  %``New Physics in $b \to s \ell^+ \ell^-$ confronts new data on Lepton Universality,''
  Eur.\ Phys.\ J.\ C {\bf 79} (2019) no.8,  719
  doi:10.1140/epjc/s10052-019-7210-9
  [arXiv:1903.09632 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-019-7210-9;%%
  %39 citations counted in INSPIRE as of 06 Oct 2019


%\cite{deMedeirosVarzielas:2019lgb}
\bibitem{deMedeirosVarzielas:2019lgb}
  I.~de Medeiros Varzielas and J.~Talbert,
  %``Simplified Models of Flavourful Leptoquarks,''
  Eur.\ Phys.\ J.\ C {\bf 79} (2019) no.6,  536
  doi:10.1140/epjc/s10052-019-7047-2
  [arXiv:1901.10484 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-019-7047-2;%%
  %5 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Gripaios:2014tna}
\bibitem{Gripaios:2014tna}
  B.~Gripaios, M.~Nardecchia and S.~A.~Renner,
  %``Composite leptoquarks and anomalies in $B$-meson decays,''
  JHEP {\bf 1505} (2015) 006
  doi:10.1007/JHEP05(2015)006
  [arXiv:1412.1791 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP05(2015)006;%%
  %197 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Varzielas:2015iva}
\bibitem{Varzielas:2015iva}
  I.~de Medeiros Varzielas and G.~Hiller,
  %``Clues for flavor from rare lepton and quark decays,''
  JHEP {\bf 1506} (2015) 072
  doi:10.1007/JHEP06(2015)072
  [arXiv:1503.01084 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP06(2015)072;%%
  %141 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Gripaios:2015gra}
\bibitem{Gripaios:2015gra}
  B.~Gripaios, M.~Nardecchia and S.~A.~Renner,
  %``Linear flavour violation and anomalies in B physics,''
  JHEP {\bf 1606} (2016) 083
  doi:10.1007/JHEP06(2016)083
  [arXiv:1509.05020 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP06(2016)083;%%
  %59 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Bauer:2015knc}
\bibitem{Bauer:2015knc}
  M.~Bauer and M.~Neubert,
  %``Minimal Leptoquark Explanation for the R$_{D^{(*)}}$ , R$_K$ , and $(g-2)_g$ Anomalies,''
  Phys.\ Rev.\ Lett.\  {\bf 116} (2016) no.14,  141802
  doi:10.1103/PhysRevLett.116.141802
  [arXiv:1511.01900 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.116.141802;%%
  %271 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Arnan:2016cpy}
\bibitem{Arnan:2016cpy}
  P.~Arnan, L.~Hofer, F.~Mescia and A.~Crivellin,
  %``Loop effects of heavy new scalars and fermions in $b\to s\mu^+\mu^-$,''
  JHEP {\bf 1704} (2017) 043
  doi:10.1007/JHEP04(2017)043
  [arXiv:1608.07832 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP04(2017)043;%%
  %60 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Hiller:2016kry}
\bibitem{Hiller:2016kry}
  G.~Hiller, D.~Loose and K.~Schönwald,
  %``Leptoquark Flavor Patterns & B Decay Anomalies,''
  JHEP {\bf 1612} (2016) 027
  doi:10.1007/JHEP12(2016)027
  [arXiv:1609.08895 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP12(2016)027;%%
  %98 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Crivellin:2016ejn}
\bibitem{Crivellin:2016ejn}
  A.~Crivellin, J.~Fuentes-Martin, A.~Greljo and G.~Isidori,
  %``Lepton Flavor Non-Universality in B decays from Dynamical Yukawas,''
  Phys.\ Lett.\ B {\bf 766} (2017) 77
  doi:10.1016/j.physletb.2016.12.057
  [arXiv:1611.02703 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2016.12.057;%%
  %67 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Crivellin:2017zlb}
\bibitem{Crivellin:2017zlb}
  A.~Crivellin, D.~Müller and T.~Ota,
  %``Simultaneous explanation of R(D$^{(∗)}$) and b→sμ$^{+}$ μ$^{−}$: the last scalar leptoquarks standing,''
  JHEP {\bf 1709} (2017) 040
  doi:10.1007/JHEP09(2017)040
  [arXiv:1703.09226 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP09(2017)040;%%
  %160 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Alonso:2017bff}
\bibitem{Alonso:2017bff}
  R.~Alonso, P.~Cox, C.~Han and T.~T.~Yanagida,
  %``Anomaly-free local horizontal symmetry and anomaly-full rare B-decays,''
  Phys.\ Rev.\ D {\bf 96} (2017) no.7,  071701
  doi:10.1103/PhysRevD.96.071701
  [arXiv:1704.08158 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.96.071701;%%
  %47 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Bonilla:2017lsq}
\bibitem{Bonilla:2017lsq}
  C.~Bonilla, T.~Modak, R.~Srivastava and J.~W.~F.~Valle,
  %``$U(1)_{B_3-3L_\mu}$ gauge symmetry as a simple description of $b\to s$ anomalies,''
  Phys.\ Rev.\ D {\bf 98} (2018) no.9,  095002
  doi:10.1103/PhysRevD.98.095002
  [arXiv:1705.00915 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.98.095002;%%
  %54 citations counted in INSPIRE as of 06 Oct 2019


%\cite{King:2017anf}
\bibitem{King:2017anf}
  S.~F.~King,
  %``Flavourful Z$^{′}$ models for $ {R}_{K^{\left(\ast \right)}} $,''
  JHEP {\bf 1708} (2017) 019
  doi:10.1007/JHEP08(2017)019
  [arXiv:1706.06100 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2017)019;%%
  %40 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Aloni:2017ixa}
\bibitem{Aloni:2017ixa}
  D.~Aloni, A.~Dery, C.~Frugiuele and Y.~Nir,
  %``Testing minimal flavor violation in leptoquark models of the $ {R_K}_{{}^{\left(\ast \right)}} $ anomaly,''
  JHEP {\bf 1711} (2017) 109
  doi:10.1007/JHEP11(2017)109
  [arXiv:1708.06161 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP11(2017)109;%%
  %23 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Assad:2017iib}
\bibitem{Assad:2017iib}
  N.~Assad, B.~Fornal and B.~Grinstein,
  %``Baryon Number and Lepton Universality Violation in Leptoquark and Diquark Models,''
  Phys.\ Lett.\ B {\bf 777} (2018) 324
  doi:10.1016/j.physletb.2017.12.042
  [arXiv:1708.06350 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2017.12.042;%%
  %98 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Calibbi:2017qbu}
\bibitem{Calibbi:2017qbu}
  L.~Calibbi, A.~Crivellin and T.~Li,
  %``Model of vector leptoquarks in view of the $B$-physics anomalies,''
  Phys.\ Rev.\ D {\bf 98} (2018) no.11,  115002
  doi:10.1103/PhysRevD.98.115002
  [arXiv:1709.00692 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.98.115002;%%
  %110 citations counted in INSPIRE as of 06 Oct 2019


%\cite{deMedeirosVarzielas:2018bcy}
\bibitem{deMedeirosVarzielas:2018bcy}
  I.~de Medeiros Varzielas and S.~F.~King,
  %``$ {R}_{K^{\left(*\right)}} $ with leptoquarks and the origin of Yukawa couplings,''
  JHEP {\bf 1811} (2018) 100
  doi:10.1007/JHEP11(2018)100
  [arXiv:1807.06023 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP11(2018)100;%%
  %13 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Grinstein:2018fgb}
\bibitem{Grinstein:2018fgb}
  B.~Grinstein, S.~Pokorski and G.~G.~Ross,
  %``Lepton non-universality in $B$ decays and fermion mass structure,''
  JHEP {\bf 1812} (2018) 079
  doi:10.1007/JHEP12(2018)079
  [arXiv:1809.01766 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP12(2018)079;%%
  %12 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Fornal:2018dqn}
\bibitem{Fornal:2018dqn}
  B.~Fornal, S.~A.~Gadam and B.~Grinstein,
  %``Left-Right SU(4) Vector Leptoquark Model for Flavor Anomalies,''
  Phys.\ Rev.\ D {\bf 99} (2019) no.5,  055025
  doi:10.1103/PhysRevD.99.055025
  [arXiv:1812.01603 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.99.055025;%%
  %24 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Allanach:2018odd}
\bibitem{Allanach:2018odd}
  B.~C.~Allanach, T.~Corbett, M.~J.~Dolan and T.~You,
  %``Hadron collider sensitivity to fat flavourful Z$^{′}$s for $ {R}_{K^{\left(\ast \right)}} $,''
  JHEP {\bf 1903} (2019) 137
  doi:10.1007/JHEP03(2019)137
  [arXiv:1810.02166 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP03(2019)137;%%
  %14 citations counted in INSPIRE as of 06 Oct 2019


%\cite{deMedeirosVarzielas:2019okf}
\bibitem{deMedeirosVarzielas:2019okf}
  I.~De Medeiros Varzielas and S.~F.~King,
  %``Origin of Yukawa couplings for Higgs bosons and leptoquarks,''
  Phys.\ Rev.\ D {\bf 99} (2019) no.9,  095029
  doi:10.1103/PhysRevD.99.095029
  [arXiv:1902.09266 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.99.095029;%%
  %4 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Allanach:2019mfl}
\bibitem{Allanach:2019mfl}
  B.~C.~Allanach, J.~M.~Butterworth and T.~Corbett,
  %``Collider constraints on Z$^{′}$ models for neutral current B-anomalies,''
  JHEP {\bf 1908} (2019) 106
  doi:10.1007/JHEP08(2019)106
  [arXiv:1904.10954 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP08(2019)106;%%
  %8 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Bordone:2017bld}
\bibitem{Bordone:2017bld}
  M.~Bordone, C.~Cornella, J.~Fuentes-Martin and G.~Isidori,
  %``A three-site gauge model for flavor hierarchies and flavor anomalies,''
  Phys.\ Lett.\ B {\bf 779} (2018) 317
  doi:10.1016/j.physletb.2018.02.011
  [arXiv:1712.01368 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2018.02.011;%%
  %89 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Bordone:2018nbg}
\bibitem{Bordone:2018nbg}
  M.~Bordone, C.~Cornella, J.~Fuentes-Martín and G.~Isidori,
  %``Low-energy signatures of the $\mathrm{PS}^3$ model: from $B$-physics anomalies to LFV,''
  JHEP {\bf 1810} (2018) 148
  doi:10.1007/JHEP10(2018)148
  [arXiv:1805.09328 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP10(2018)148;%%
  %48 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Becirevic:2018afm}
\bibitem{Becirevic:2018afm}
  D.~Bečirević, I.~Doršner, S.~Fajfer, N.~Košnik, D.~A.~Faroughy and O.~Sumensari,
  %``Scalar leptoquarks from grand unified theories to accommodate the $B$-physics anomalies,''
  Phys.\ Rev.\ D {\bf 98} (2018) no.5,  055003
  doi:10.1103/PhysRevD.98.055003
  [arXiv:1806.05689 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.98.055003;%%
  %71 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Angelescu:2018tyl}
\bibitem{Angelescu:2018tyl}
  A.~Angelescu, D.~Bečirević, D.~A.~Faroughy and O.~Sumensari,
  %``Closing the window on single leptoquark solutions to the $B$-physics anomalies,''
  JHEP {\bf 1810} (2018) 183
  doi:10.1007/JHEP10(2018)183
  [arXiv:1808.08179 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP10(2018)183;%%
  %61 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Cornella:2019hct}
\bibitem{Cornella:2019hct}
  C.~Cornella, J.~Fuentes-Martin and G.~Isidori,
  %``Revisiting the vector leptoquark explanation of the B-physics anomalies,''
  JHEP {\bf 1907} (2019) 168
  doi:10.1007/JHEP07(2019)168
  [arXiv:1903.11517 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP07(2019)168;%%
  %27 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Datta:2019tuj}
\bibitem{Datta:2019tuj}
  A.~Datta, D.~Sachdeva and J.~Waite,
  %``Unified explanation of $b \to s \mu^+ \mu^-$ anomalies, neutrino masses, and $B\rightarrow \pi K$ puzzle,''
  Phys.\ Rev.\ D {\bf 100} (2019) no.5,  055015
  doi:10.1103/PhysRevD.100.055015
  [arXiv:1905.04046 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.100.055015;%%
  %5 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Blanke:2018sro}
\bibitem{Blanke:2018sro}
  M.~Blanke and A.~Crivellin,
  %``$B$ Meson Anomalies in a Pati-Salam Model within the Randall-Sundrum Background,''
  Phys.\ Rev.\ Lett.\  {\bf 121} (2018) no.1,  011801
  doi:10.1103/PhysRevLett.121.011801
  [arXiv:1801.07256 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.121.011801;%%
  %97 citations counted in INSPIRE as of 06 Oct 2019

%\cite{Perez:2013osa}
\bibitem{Perez:2013osa} 
  P.~Fileviez Perez and M.~B.~Wise,
  %``Low Scale Quark-Lepton Unification,''
  Phys.\ Rev.\ D {\bf 88}, 057703 (2013)
  doi:10.1103/PhysRevD.88.057703
  [arXiv:1307.6213 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.057703;%%
  %27 citations counted in INSPIRE as of 09 Oct 2019


%\cite{Biggio:2016wyy}
\bibitem{Biggio:2016wyy} 
  C.~Biggio, M.~Bordone, L.~Di Luzio and G.~Ridolfi,
  %``Massive vectors and loop observables: the $g-2$ case,''
  JHEP {\bf 1610}, 002 (2016)
  doi:10.1007/JHEP10(2016)002
  [arXiv:1607.07621 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP10(2016)002;%%
  %28 citations counted in INSPIRE as of 09 Oct 2019


%\cite{Dorsner:2016wpm}
\bibitem{Dorsner:2016wpm}
  I.~Doršner, S.~Fajfer, A.~Greljo, J.~F.~Kamenik and N.~Košnik,
  %``Physics of leptoquarks in precision experiments and at particle colliders,''
  Phys.\ Rept.\  {\bf 641} (2016) 1
  doi:10.1016/j.physrep.2016.06.001
  [arXiv:1603.04993 [hep-ph]].
  %%CITATION = doi:10.1016/j.physrep.2016.06.001;%%
  %217 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Hiller:2018wbv}
\bibitem{Hiller:2018wbv}
  G.~Hiller, D.~Loose and I.~Nišandžić,
  %``Flavorful leptoquarks at hadron colliders,''
  Phys.\ Rev.\ D {\bf 97} (2018) no.7,  075004
  doi:10.1103/PhysRevD.97.075004
  [arXiv:1801.09399 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.97.075004;%%
  %19 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Diaz:2017lit}
\bibitem{Diaz:2017lit}
  B.~Diaz, M.~Schmaltz and Y.~M.~Zhong,
  %``The leptoquark Hunter’s guide: Pair production,''
  JHEP {\bf 1710} (2017) 097
  doi:10.1007/JHEP10(2017)097
  [arXiv:1706.05033 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP10(2017)097;%%
  %51 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Schmaltz:2018nls}
\bibitem{Schmaltz:2018nls}
  M.~Schmaltz and Y.~M.~Zhong,
  %``The leptoquark Hunter’s guide: large coupling,''
  JHEP {\bf 1901} (2019) 132
  doi:10.1007/JHEP01(2019)132
  [arXiv:1810.10017 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP01(2019)132;%%
  %19 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Baker:2019sli}
\bibitem{Baker:2019sli}
  M.~J.~Baker, J.~Fuentes-Martín, G.~Isidori and M.~König,
  %``High- $p_T$ signatures in vector–leptoquark models,''
  Eur.\ Phys.\ J.\ C {\bf 79} (2019) no.4,  334
  doi:10.1140/epjc/s10052-019-6853-x
  [arXiv:1901.10480 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-019-6853-x;%%
  %12 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Lam:2007qc}
\bibitem{Lam:2007qc}
  C.~S.~Lam,
  %``Symmetry of Lepton Mixing,''
  Phys.\ Lett.\ B {\bf 656} (2007) 193
  doi:10.1016/j.physletb.2007.09.032
  [arXiv:0708.3665 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2007.09.032;%%
  %158 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Ge:2011ih}
\bibitem{Ge:2011ih}
  S.~F.~Ge, D.~A.~Dicus and W.~W.~Repko,
  %``Z_2 Symmetry Prediction for the Leptonic Dirac CP Phase,''
  Phys.\ Lett.\ B {\bf 702} (2011) 220
  doi:10.1016/j.physletb.2011.06.096
  [arXiv:1104.0602 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2011.06.096;%%
  %132 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Ge:2011qn}
\bibitem{Ge:2011qn}
  S.~F.~Ge, D.~A.~Dicus and W.~W.~Repko,
  %``Residual Symmetries for Neutrino Mixing with a Large $\theta_{13}$ and Nearly Maximal $\delta_D$,''
  Phys.\ Rev.\ Lett.\  {\bf 108} (2012) 041801
  doi:10.1103/PhysRevLett.108.041801
  [arXiv:1108.0964 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevLett.108.041801;%%
  %173 citations counted in INSPIRE as of 06 Oct 2019


%\cite{deAdelhartToorop:2011re}
\bibitem{deAdelhartToorop:2011re}
  R.~de Adelhart Toorop, F.~Feruglio and C.~Hagedorn,
  %``Finite Modular Groups and Lepton Mixing,''
  Nucl.\ Phys.\ B {\bf 858} (2012) 437
  doi:10.1016/j.nuclphysb.2012.01.017
  [arXiv:1112.1340 [hep-ph]].
  %%CITATION = doi:10.1016/j.nuclphysb.2012.01.017;%%
  %161 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Hernandez:2012ra}
\bibitem{Hernandez:2012ra}
  D.~Hernandez and A.~Y.~Smirnov,
  %``Lepton mixing and discrete symmetries,''
  Phys.\ Rev.\ D {\bf 86} (2012) 053014
  doi:10.1103/PhysRevD.86.053014
  [arXiv:1204.0445 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.86.053014;%%
  %157 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Lam:2012ga}
\bibitem{Lam:2012ga}
  C.~S.~Lam,
  %``Finite Symmetry of Leptonic Mass Matrices,''
  Phys.\ Rev.\ D {\bf 87} (2013) no.1,  013001
  doi:10.1103/PhysRevD.87.013001
  [arXiv:1208.5527 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.87.013001;%%
  %62 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Holthausen:2012wt}
\bibitem{Holthausen:2012wt}
  M.~Holthausen, K.~S.~Lim and M.~Lindner,
  %``Lepton Mixing Patterns from a Scan of Finite Discrete Groups,''
  Phys.\ Lett.\ B {\bf 721} (2013) 61
  doi:10.1016/j.physletb.2013.02.047
  [arXiv:1212.2411 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2013.02.047;%%
  %93 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Holthausen:2013vba}
\bibitem{Holthausen:2013vba}
  M.~Holthausen and K.~S.~Lim,
  %``Quark and Leptonic Mixing Patterns from the Breakdown of a Common Discrete Flavor Symmetry,''
  Phys.\ Rev.\ D {\bf 88} (2013) 033018
  doi:10.1103/PhysRevD.88.033018
  [arXiv:1306.4356 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.88.033018;%%
  %57 citations counted in INSPIRE as of 06 Oct 2019


%\cite{King:2013vna}
\bibitem{King:2013vna}
  S.~F.~King, T.~Neder and A.~J.~Stuart,
  %``Lepton mixing predictions from $\Delta(6n^2)$ family Symmetry,''
  Phys.\ Lett.\ B {\bf 726} (2013) 312
  doi:10.1016/j.physletb.2013.08.052
  [arXiv:1305.3200 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2013.08.052;%%
  %94 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Lavoura:2014kwa}
\bibitem{Lavoura:2014kwa}
  L.~Lavoura and P.~O.~Ludl,
  %``Residual $\mathbb{Z}_2 \times \mathbb{Z}_2$ symmetries and lepton mixing,''
  Phys.\ Lett.\ B {\bf 731} (2014) 331
  doi:10.1016/j.physletb.2014.03.001
  [arXiv:1401.5036 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2014.03.001;%%
  %25 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Fonseca:2014koa}
\bibitem{Fonseca:2014koa}
  R.~M.~Fonseca and W.~Grimus,
  %``Classification of lepton mixing matrices from finite residual symmetries,''
  JHEP {\bf 1409} (2014) 033
  doi:10.1007/JHEP09(2014)033
  [arXiv:1405.3678 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP09(2014)033;%%
  %82 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Hu:2014kca}
\bibitem{Hu:2014kca}
  B.~Hu,
  %``Lepton Mixing, Residual Symmetries, and Trigonometric Diophantine Equations,''
  Phys.\ Rev.\ D {\bf 90} (2014) no.7,  073012
  doi:10.1103/PhysRevD.90.073012
  [arXiv:1407.4722 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.073012;%%
  %6 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Joshipura:2014pqa}
\bibitem{Joshipura:2014pqa}
  A.~S.~Joshipura and K.~M.~Patel,
  %``A massless neutrino and lepton mixing patterns from finite discrete subgroups of U(3),''
  JHEP {\bf 1404} (2014) 009
  doi:10.1007/JHEP04(2014)009
  [arXiv:1401.6397 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP04(2014)009;%%
  %16 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Joshipura:2014qaa}
\bibitem{Joshipura:2014qaa}
  A.~S.~Joshipura and K.~M.~Patel,
  %``Discrete flavor symmetries for degenerate solar neutrino pair and their predictions,''
  Phys.\ Rev.\ D {\bf 90} (2014) no.3,  036005
  doi:10.1103/PhysRevD.90.036005
  [arXiv:1405.6106 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.90.036005;%%
  %18 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Talbert:2014bda}
\bibitem{Talbert:2014bda}
  J.~Talbert,
  %``[Re]constructing Finite Flavour Groups: Horizontal Symmetry Scans from the Bottom-Up,''
  JHEP {\bf 1412} (2014) 058
  doi:10.1007/JHEP12(2014)058
  [arXiv:1409.7310 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP12(2014)058;%%
  %27 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Yao:2015dwa}
\bibitem{Yao:2015dwa}
  C.~Y.~Yao and G.~J.~Ding,
  %``Lepton and Quark Mixing Patterns from Finite Flavor Symmetries,''
  Phys.\ Rev.\ D {\bf 92} (2015) no.9,  096010
  doi:10.1103/PhysRevD.92.096010
  [arXiv:1505.03798 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.92.096010;%%
  %37 citations counted in INSPIRE as of 06 Oct 2019


%\cite{King:2016pgv}
\bibitem{King:2016pgv}
  S.~F.~King and P.~O.~Ludl,
  %``Direct and Semi-Direct Approaches to Lepton Mixing with a Massless Neutrino,''
  JHEP {\bf 1606} (2016) 147
  doi:10.1007/JHEP06(2016)147
  [arXiv:1605.01683 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP06(2016)147;%%
  %13 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Varzielas:2016zuo}
\bibitem{Varzielas:2016zuo}
  I.~de Medeiros Varzielas, R.~W.~Rasmussen and J.~Talbert,
  %``Bottom-Up Discrete Symmetries for Cabibbo Mixing,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 32} (2017) no.06n07,  1750047
  doi:10.1142/S0217751X17500476
  [arXiv:1605.03581 [hep-ph]].
  %%CITATION = doi:10.1142/S0217751X17500476;%%
  %18 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Yao:2016zev}
\bibitem{Yao:2016zev}
  C.~Y.~Yao and G.~J.~Ding,
  %``CP Symmetry and Lepton Mixing from a Scan of Finite Discrete Groups,''
  Phys.\ Rev.\ D {\bf 94} (2016) no.7,  073006
  doi:10.1103/PhysRevD.94.073006
  [arXiv:1606.05610 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.94.073006;%%
  %26 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Lu:2016jit}
\bibitem{Lu:2016jit}
  J.~N.~Lu and G.~J.~Ding,
  %``Alternative Schemes of Predicting Lepton Mixing Parameters from Discrete Flavor and CP Symmetry,''
  Phys.\ Rev.\ D {\bf 95} (2017) no.1,  015012
  doi:10.1103/PhysRevD.95.015012
  [arXiv:1610.05682 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.95.015012;%%
  %21 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Li:2017abz}
\bibitem{Li:2017abz}
  C.~C.~Li, J.~N.~Lu and G.~J.~Ding,
  %``Toward a unified interpretation of quark and lepton mixing from flavor and CP symmetries,''
  JHEP {\bf 1802} (2018) 038
  doi:10.1007/JHEP02(2018)038
  [arXiv:1706.04576 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP02(2018)038;%%
  %13 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Lu:2018oxc}
\bibitem{Lu:2018oxc}
  J.~N.~Lu and G.~J.~Ding,
  %``Quark and lepton mixing patterns from a common discrete flavor symmetry with a generalized CP symmetry,''
  Phys.\ Rev.\ D {\bf 98} (2018) no.5,  055011
  doi:10.1103/PhysRevD.98.055011
  [arXiv:1806.02301 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.98.055011;%%
  %12 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Hagedorn:2018gpw}
\bibitem{Hagedorn:2018gpw}
  C.~Hagedorn and J.~König,
  %``Lepton and Quark Mixing from Stepwise Breaking of Flavor and CP,''
  arXiv:1811.07750 [hep-ph].
  %%CITATION = ARXIV:1811.07750;%%
  %7 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Lu:2019gqp}
\bibitem{Lu:2019gqp}
  J.~N.~Lu and G.~J.~Ding,
  %``Dihedral flavor group as the key to understand quark and lepton flavor mixing,''
  JHEP {\bf 1903} (2019) 056
  doi:10.1007/JHEP03(2019)056
  [arXiv:1901.07414 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP03(2019)056;%%
  %7 citations counted in INSPIRE as of 06 Oct 2019


%\cite{King:2013eh}
\bibitem{King:2013eh}
  S.~F.~King and C.~Luhn,
  %``Neutrino Mass and Mixing with Discrete Symmetry,''
  Rept.\ Prog.\ Phys.\  {\bf 76} (2013) 056201
  doi:10.1088/0034-4885/76/5/056201
  [arXiv:1301.1340 [hep-ph]].
  %%CITATION = doi:10.1088/0034-4885/76/5/056201;%%
  %527 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Altarelli:2010gt}
\bibitem{Altarelli:2010gt}
  G.~Altarelli and F.~Feruglio,
  %``Discrete Flavor Symmetries and Models of Neutrino Mixing,''
  Rev.\ Mod.\ Phys.\  {\bf 82} (2010) 2701
  doi:10.1103/RevModPhys.82.2701
  [arXiv:1002.0211 [hep-ph]].
  %%CITATION = doi:10.1103/RevModPhys.82.2701;%%
  %698 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Grimus:2011fk}
\bibitem{Grimus:2011fk}
  W.~Grimus and P.~O.~Ludl,
  %``Finite flavour groups of fermions,''
  J.\ Phys.\ A {\bf 45} (2012) 233001
  doi:10.1088/1751-8113/45/23/233001
  [arXiv:1110.6376 [hep-ph]].
  %%CITATION = doi:10.1088/1751-8113/45/23/233001;%%
  %124 citations counted in INSPIRE as of 06 Oct 2019

%\cite{Sch97}
\bibitem{Sch97}
         Martin Sch{\accent127 o}nert et~al.
 \newblock {\em {GAP} --
         {Groups}, {Algorithms}, and {Programming} --
       version 3 release 4 patchlevel 4"}.
\newblock Lehrstuhl D f{\accent127 u}r Mathematik,
       Rheinisch Westf{\accent127 a}lische
     Technische Hoch\-schule, Aachen, Germany, 1997.

%\cite{GAP4}
\bibitem{GAP4}
 The GAP~Group, \emph{GAP -- Groups, Algorithms, and Programming, 
 Version 4.10.1}; 
 2019,
  \verb+(https://www.gap-system.org)+.


%\cite{Minkowski:1977sc}
\bibitem{Minkowski:1977sc}
  P.~Minkowski,
  %``$\mu \to e\gamma$ at a Rate of One Out of $10^{9}$ Muon Decays?,''
  Phys.\ Lett.\  {\bf 67B} (1977) 421.
  doi:10.1016/0370-2693(77)90435-X
  %%CITATION = doi:10.1016/0370-2693(77)90435-X;%%
  %3528 citations counted in INSPIRE as of 06 Oct 2019


%\cite{deMedeirosVarzielas:2017sdv}
\bibitem{deMedeirosVarzielas:2017sdv}
  I.~de Medeiros Varzielas, G.~G.~Ross and J.~Talbert,
  %``A Unified Model of Quarks and Leptons with a Universal Texture Zero,''
  JHEP {\bf 1803} (2018) 007
  doi:10.1007/JHEP03(2018)007
  [arXiv:1710.01741 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP03(2018)007;%%
  %21 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Altarelli:2005yx}
\bibitem{Altarelli:2005yx}
  G.~Altarelli and F.~Feruglio,
  %``Tri-bimaximal neutrino mixing, A(4) and the modular symmetry,''
  Nucl.\ Phys.\ B {\bf 741} (2006) 215
  doi:10.1016/j.nuclphysb.2006.02.015
  [hep-ph/0512103].
  %%CITATION = doi:10.1016/j.nuclphysb.2006.02.015;%%
  %598 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Harrison:2002er}
\bibitem{Harrison:2002er}
  P.~F.~Harrison, D.~H.~Perkins and W.~G.~Scott,
  %``Tri-bimaximal mixing and the neutrino oscillation data,''
  Phys.\ Lett.\ B {\bf 530} (2002) 167
  doi:10.1016/S0370-2693(02)01336-9
  [hep-ph/0202074].
  %%CITATION = doi:10.1016/S0370-2693(02)01336-9;%%
  %1432 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Davidson:1993qk}
\bibitem{Davidson:1993qk}
  S.~Davidson, D.~C.~Bailey and B.~A.~Campbell,
  %``Model independent constraints on leptoquarks from rare processes,''
  Z.\ Phys.\ C {\bf 61} (1994) 613
  doi:10.1007/BF01552629
  [hep-ph/9309310].
  %%CITATION = doi:10.1007/BF01552629;%%
  %452 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Gonzalez-Alonso:2017iyc}
\bibitem{Gonzalez-Alonso:2017iyc}
  M.~Gonz{\'a}lez-Alonso, J.~Martin Camalich and K.~Mimouni,
  %``Renormalization-group evolution of new physics contributions to (semi)leptonic meson decays,''
  Phys.\ Lett.\ B {\bf 772} (2017) 777
  doi:10.1016/j.physletb.2017.07.003
  [arXiv:1706.00410 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2017.07.003;%%
  %48 citations counted in INSPIRE as of 08 Jan 2020

%\cite{Crivellin:2019kps}
\bibitem{Crivellin:2019kps}
  A.~Crivellin and F.~Saturnino,
  %``Correlating tauonic $B$ decays with the neutron electric dipole moment via a scalar leptoquark,''
  Phys.\ Rev.\ D {\bf 100} (2019) no.11,  115014
  doi:10.1103/PhysRevD.100.115014
  [arXiv:1905.08257 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.100.115014;%%
  %8 citations counted in INSPIRE as of 08 Jan 2020

%\cite{Dekens:2018bci}
\bibitem{Dekens:2018bci}
  W.~Dekens, J.~de Vries, M.~Jung and K.~K.~Vos,
  %``The phenomenology of electric dipole moments in models of scalar leptoquarks,''
  JHEP {\bf 1901} (2019) 069
  doi:10.1007/JHEP01(2019)069
  [arXiv:1809.09114 [hep-ph]].
  %%CITATION = doi:10.1007/JHEP01(2019)069;%%
  %26 citations counted in INSPIRE as of 08 Jan 2020

%\cite{Kumar:2018kmr}
\bibitem{Kumar:2018kmr}
  J.~Kumar, D.~London and R.~Watanabe,
  %``Combined Explanations of the $b \to s \mu^+ \mu^-$ and $b \to c \tau^- {\bar\nu}$ Anomalies: a General Model Analysis,''
  Phys.\ Rev.\ D {\bf 99} (2019) no.1,  015007
  doi:10.1103/PhysRevD.99.015007
  [arXiv:1806.07403 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.99.015007;%%
  %55 citations counted in INSPIRE as of 08 Jan 2020


%\cite{Olechowski:1990bh}
\bibitem{Olechowski:1990bh}
  M.~Olechowski and S.~Pokorski,
  %``Heavy top quark and scale dependence of quark mixing,''
  Phys.\ Lett.\ B {\bf 257} (1991) 388.
  doi:10.1016/0370-2693(91)91912-F
  %%CITATION = doi:10.1016/0370-2693(91)91912-F;%%
  %82 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Ross:2007az}
\bibitem{Ross:2007az}
  G.~Ross and M.~Serna,
  %``Unification and fermion mass structure,''
  Phys.\ Lett.\ B {\bf 664} (2008) 97
  doi:10.1016/j.physletb.2008.05.014
  [arXiv:0704.1248 [hep-ph]].
  %%CITATION = doi:10.1016/j.physletb.2008.05.014;%%
  %128 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Varzielas:2008jm}
\bibitem{Varzielas:2008jm}
  I.~de Medeiros Varzielas, G.~G.~Ross and M.~Serna,
  %``Quasi-degenerate neutrinos and tri-bi-maximal mixing,''
  Phys.\ Rev.\ D {\bf 80} (2009) 073002
  doi:10.1103/PhysRevD.80.073002
  [arXiv:0811.2226 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.80.073002;%%
  %24 citations counted in INSPIRE as of 10 Oct 2019


%\cite{Chiu:2016qra}
\bibitem{Chiu:2016qra}
  S.~H.~Chiu and T.~K.~Kuo,
  %``Renormalization of the quark mass matrix,''
  Phys.\ Rev.\ D {\bf 93} (2016) no.9,  093006
  doi:10.1103/PhysRevD.93.093006
  [arXiv:1603.04568 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.93.093006;%%
  %6 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Casas:1999tg}
\bibitem{Casas:1999tg}
  J.~A.~Casas, J.~R.~Espinosa, A.~Ibarra and I.~Navarro,
  %``General RG equations for physical neutrino parameters and their phenomenological implications,''
  Nucl.\ Phys.\ B {\bf 573} (2000) 652
  doi:10.1016/S0550-3213(99)00781-6
  [hep-ph/9910420].
  %%CITATION = doi:10.1016/S0550-3213(99)00781-6;%%
  %230 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Casas:1999ac}
\bibitem{Casas:1999ac}
  J.~A.~Casas, J.~R.~Espinosa, A.~Ibarra and I.~Navarro,
  %``Nearly degenerate neutrinos, supersymmetry and radiative corrections,''
  Nucl.\ Phys.\ B {\bf 569} (2000) 82
  doi:10.1016/S0550-3213(99)00605-7
  [hep-ph/9905381].
  %%CITATION = doi:10.1016/S0550-3213(99)00605-7;%%
  %184 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Chankowski:1999xc}
\bibitem{Chankowski:1999xc}
  P.~H.~Chankowski, W.~Krolikowski and S.~Pokorski,
  %``Fixed points in the evolution of neutrino mixings,''
  Phys.\ Lett.\ B {\bf 473} (2000) 109
  doi:10.1016/S0370-2693(99)01465-3
  [hep-ph/9910231].
  %%CITATION = doi:10.1016/S0370-2693(99)01465-3;%%
  %130 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Antusch:2003kp}
\bibitem{Antusch:2003kp}
  S.~Antusch, J.~Kersten, M.~Lindner and M.~Ratz,
  %``Running neutrino masses, mixings and CP phases: Analytical results and phenomenological consequences,''
  Nucl.\ Phys.\ B {\bf 674} (2003) 401
  doi:10.1016/j.nuclphysb.2003.09.050
  [hep-ph/0305273].
  %%CITATION = doi:10.1016/j.nuclphysb.2003.09.050;%%
  %335 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Datta:2003qg}
\bibitem{Datta:2003qg}
  A.~Datta, F.~S.~Ling and P.~Ramond,
  %``Correlated hierarchy, Dirac masses and large mixing angles,''
  Nucl.\ Phys.\ B {\bf 671} (2003) 383
  doi:10.1016/j.nuclphysb.2003.08.026
  [hep-ph/0306002].
  %%CITATION = doi:10.1016/j.nuclphysb.2003.08.026;%%
  %110 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Adulpravitchai:2009bg}
\bibitem{Adulpravitchai:2009bg}
  A.~Adulpravitchai, A.~Blum and W.~Rodejohann,
  %``Golden Ratio Prediction for Solar Neutrino Mixing,''
  New J.\ Phys.\  {\bf 11} (2009) 063026
  doi:10.1088/1367-2630/11/6/063026
  [arXiv:0903.0531 [hep-ph]].
  %%CITATION = doi:10.1088/1367-2630/11/6/063026;%%
  %81 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Fukugita:1998vn}
\bibitem{Fukugita:1998vn}
  M.~Fukugita, M.~Tanimoto and T.~Yanagida,
  %``Atmospheric neutrino oscillation and a phenomenological lepton mass matrix,''
  Phys.\ Rev.\ D {\bf 57} (1998) 4429
  doi:10.1103/PhysRevD.57.4429
  [hep-ph/9709388].
  %%CITATION = doi:10.1103/PhysRevD.57.4429;%%
  %254 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Giunti:2002sr}
\bibitem{Giunti:2002sr}
  C.~Giunti,
  %``Current status of neutrino masses and mixings,''
  Nucl.\ Phys.\ Proc.\ Suppl.\  {\bf 117} (2003) 24
  doi:10.1016/S0920-5632(03)90480-4
  [hep-ph/0209103].
  %%CITATION = doi:10.1016/S0920-5632(03)90480-4;%%
  %32 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Albright:2010ap}
\bibitem{Albright:2010ap}
  C.~H.~Albright, A.~Dueck and W.~Rodejohann,
  %``Possible Alternatives to Tri-bimaximal Mixing,''
  Eur.\ Phys.\ J.\ C {\bf 70} (2010) 1099
  doi:10.1140/epjc/s10052-010-1492-2
  [arXiv:1004.2798 [hep-ph]].
  %%CITATION = doi:10.1140/epjc/s10052-010-1492-2;%%
  %173 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Ishimori:2010au}
\bibitem{Ishimori:2010au}
  H.~Ishimori, T.~Kobayashi, H.~Ohki, Y.~Shimizu, H.~Okada and M.~Tanimoto,
  %``Non-Abelian Discrete Symmetries in Particle Physics,''
  Prog.\ Theor.\ Phys.\ Suppl.\  {\bf 183} (2010) 1
  doi:10.1143/PTPS.183.1
  [arXiv:1003.3552 [hep-th]].
  %%CITATION = doi:10.1143/PTPS.183.1;%%
  %635 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Blum:2007jz}
\bibitem{Blum:2007jz}
  A.~Blum, C.~Hagedorn and M.~Lindner,
  %``Fermion Masses and Mixings from Dihedral Flavor Symmetries with Preserved Subgroups,''
  Phys.\ Rev.\ D {\bf 77} (2008) 076004
  doi:10.1103/PhysRevD.77.076004
  [arXiv:0709.3450 [hep-ph]].
  %%CITATION = doi:10.1103/PhysRevD.77.076004;%%
  %122 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Lees:2012xj}
\bibitem{Lees:2012xj}
  J.~P.~Lees {\it et al.} [BaBar Collaboration],
  %``Evidence for an excess of $\bar{B} \to D^{(*)} \tau^-\bar{\nu}_\tau$ decays,''
  Phys.\ Rev.\ Lett.\  {\bf 109} (2012) 101802
  doi:10.1103/PhysRevLett.109.101802
  [arXiv:1205.5442 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.109.101802;%%
  %717 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Lees:2013uzd}
\bibitem{Lees:2013uzd}
  J.~P.~Lees {\it et al.} [BaBar Collaboration],
  %``Measurement of an Excess of $\bar{B} \to D^{(*)}\tau^- \bar{\nu}_\tau$ Decays and Implications for Charged Higgs Bosons,''
  Phys.\ Rev.\ D {\bf 88} (2013) no.7,  072012
  doi:10.1103/PhysRevD.88.072012
  [arXiv:1303.0571 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevD.88.072012;%%
  %586 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Huschle:2015rga}
\bibitem{Huschle:2015rga}
  M.~Huschle {\it et al.} [Belle Collaboration],
  %``Measurement of the branching ratio of $\bar{B} \to D^{(\ast)} \tau^- \bar{\nu}_\tau$ relative to $\bar{B} \to D^{(\ast)} \ell^- \bar{\nu}_\ell$ decays with hadronic tagging at Belle,''
  Phys.\ Rev.\ D {\bf 92} (2015) no.7,  072014
  doi:10.1103/PhysRevD.92.072014
  [arXiv:1507.03233 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevD.92.072014;%%
  %538 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Aaij:2015yra}
\bibitem{Aaij:2015yra}
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Measurement of the ratio of branching fractions $\mathcal{B}(\bar{B}^0 \to D^{*+}\tau^{-}\bar{\nu}_{\tau})/\mathcal{B}(\bar{B}^0 \to D^{*+}\mu^{-}\bar{\nu}_{\mu})$,''
  Phys.\ Rev.\ Lett.\  {\bf 115} (2015) no.11,  111803
   Erratum: [Phys.\ Rev.\ Lett.\  {\bf 115} (2015) no.15,  159901]
  doi:10.1103/PhysRevLett.115.159901, 10.1103/PhysRevLett.115.111803
  [arXiv:1506.08614 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.115.159901, 10.1103/PhysRevLett.115.111803;%%
  %654 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Hirose:2016wfn}
\bibitem{Hirose:2016wfn}
  S.~Hirose {\it et al.} [Belle Collaboration],
  %``Measurement of the $\tau$ lepton polarization and $R(D^*)$ in the decay $\bar{B} \to D^* \tau^- \bar{\nu}_\tau$,''
  Phys.\ Rev.\ Lett.\  {\bf 118} (2017) no.21,  211801
  doi:10.1103/PhysRevLett.118.211801
  [arXiv:1612.00529 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevLett.118.211801;%%
  %302 citations counted in INSPIRE as of 06 Oct 2019


%\cite{Aaij:2017deq}
\bibitem{Aaij:2017deq}
  R.~Aaij {\it et al.} [LHCb Collaboration],
  %``Test of Lepton Flavor Universality by the measurement of the $B^0 \to D^{*-} \tau^+ \nu_{\tau}$ branching fraction using three-prong $\tau$ decays,''
  Phys.\ Rev.\ D {\bf 97} (2018) no.7,  072013
  doi:10.1103/PhysRevD.97.072013
  [arXiv:1711.02505 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevD.97.072013;%%
  %122 citations counted in INSPIRE as of 06 Oct 2019

  %\cite{Moriond2019}
\bibitem{Moriond2019BelleRD}
G. Caria, talk at 2019 Rencontres de Moriond, Electroweak Interactions and Unified Theories, http://moriond.in2p3.fr/2019/EW

